Analysis of EUV Solar Spectrum with Gravity Induced Resonant Emission

Gravity Induced Resonant Emission (GIRE) is a new phenomenon recently reported; we have analyzed the solar emissions on the basis of GIRE. We have computed the EUV solar spectrum using GIRE wave length as a part of studying coronal heating problem. We find all the solar observations converge in GIRE and the GIRE wave length is sufficient to study all the solar emissions.

==> LaTeX1table.tex <==
\begin{table}
\begin{tabular}{||l|lr||} \hline
\textbf{Veg}  & \multicolumn{2}{|c||}{\textbf{Detail}}\\\hline
carrots    & per pound & \pounds 0.75 \\ \cline{2-3}
					 & each      &         20p  \\ \hline
mushrooms  & dozen     &         86p  \\ \cline{1-1} \cline{3-3}
toadstools & pick your own & free     \\ \hline
\end{tabular}
\end{table}

==> arXive EUV/LaTeX1table.tex <==
\begin{table}
\begin{tabular}{||l|lr||} \hline
\textbf{Veg}  & \multicolumn{2}{|c||}{\textbf{Detail}}\\\hline
carrots    & per pound & \pounds 0.75 \\ \cline{2-3}
					 & each      &         20p  \\ \hline
mushrooms  & dozen     &         86p  \\ \cline{1-1} \cline{3-3}
toadstools & pick your own & free     \\ \hline
\end{tabular}
\end{table}

==> arXive EUV/table2.tex <==



==> table2.tex <==


